Automating Compliance in Government Organisations using eFLINT

Ensuring compliance of norms and policies when working on administrative law cases can be difficult to manage for government organisations. Automating this process could save a lot of time, effort and ensure compliance. Prior research resulted in a method to formalize sources of norms. These can be turned into executable specifications using the domain-specific language eFLINT, which can be used for automating compliance. However, the current interface of eFLINT prevents adaption by legal experts. The aim of this research was to bridge this gap by developing a prototype based on eFLINT, for automating compliance within government organisations. To get a better understanding of the needs and requirements of potential users, qualitative research was conducted. This consisted of semi-structured interviews to gather requirements, which were analyzed using a thematic analysis method. Based on the analyzed data, a design for the interface of the prototype was made. The final prototype was evaluated in a user end study which included a cognitive walkthrough and user testing. The prototype proved to be a good first step in the right direction with a lot of room for further development.

==> titlepage.tex <==
\begin{center}
 
\textsc{\Huge Automating Compliance in Government Organisations using eFLINT}

\bigskip
\bigskip

\textsc{\large
submitted in partial fulfillment for the degree of master of science\\
%
\bigskip
\bigskip
Nina Verheijen\\
%
11764198\\
%
\bigskip
\bigskip
master information studies\\
%
Information Systems\\
%
faculty of science\\
%
university of amsterdam\\
%
\bigskip
\bigskip
% fill in your date of defence in format yyyy-mm-dd
}

%if you want to have a cover image (for example the most interesting figure of the thesis), then please un-comment the two lines below and replace it with your own image

%\vfill

%\includegraphics[width=.5\paperwidth]{titlepage-media/logo-uva.png} 
 
\vfill

\begin{tabular}{lll}
  \textbf{1st Examiner} & \textbf{2nd Examiner}  \\   
title and name of 1st Examiner & title and name of 2nd Examiner \\
affiliations of 1st Examiner & affiliations of 2nd Examiner \\ 
email of 1st Examiner & email of 2nd Examiner \\
\end{tabular}

\vfill

% if you want to include logos from your company or research group you can copy and pase the line below and replace it with your logos

\includegraphics[width=.1\paperwidth]{titlepage-media/logo-uva.png} 
%\includegraphics[width=.5\paperwidth]{titlepage-media/company-logo.png} 

\end{center}

